The Dark Side of the Web: Towards Understanding Various Data Sources in Cyber Threat Intelligence

Cyber threats have become increasingly prevalent and sophisticated. Prior work has extracted actionable cyber threat intelligence (CTI), such as indicators of compromise, tactics, techniques, and procedures (TTPs), or threat feeds from various sources: open source data (e.g., social networks), internal intelligence (e.g., log data), and ``first-hand'' communications from cybercriminals (e.g., underground forums, chats, darknet websites). However, "first-hand" data sources remain underutilized because it is difficult to access or scrape their data. In this work, we analyze (i) 6.6 million posts, (ii) 3.4 million messages, and (iii) 120,000 darknet websites. We combine NLP tools to address several challenges in analyzing such data. First, even on dedicated platforms, only some content is CTI-relevant, requiring effective filtering. Second, "first-hand" data can be CTI-relevant from a technical or strategic viewpoint. We demonstrate how to organize content along this distinction. Third, we describe the topics discussed and how "first-hand" data sources differ from each other. According to our filtering, 20% of our sample is CTI-relevant. Most of the CTI-relevant data focuses on strategic rather than technical discussions. Credit card-related crime is the most prevalent topic on darknet websites. On underground forums and chat channels, account and subscription selling is discussed most. Topic diversity is higher on underground forums and chat channels than on darknet websites. Our analyses suggest that different platforms may be used for activities with varying complexity and risks for criminals.

==> Scripts/sankey-chart-code.tex <==
All data [179952] Non-Technical
All data [15512] Technical
All data [16536] Technical + Non-Technical

Technical + Non-Technical [4520]  MITRE 
Technical + Non-Technical [10720]  Regex 
Technical + Non-Technical [1296]  MITRE + Regex 

Technical [9042]  MITRE 
Technical [6331]  Regex 
Technical [139]  MITRE + Regex 


Non-Technical [18733] Account/Accounts
Non-Technical [11112] Server
Non-Technical [6654] Code
Non-Technical [5553] Banned
Non-Technical [4567] Attack
//Non-Technical [3842] Bot
//Non-Technical [3834] Ban
//Non-Technical [3817] Fake
//Non-Technical [3216] Script
//Non-Technical [3031] File


==> figures/archived/table_rel_work.tex <==
\begin{table}
\centering
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[50]Q[55]Q[260]Q[50]Q[212]Q[80]},
  hlines,
  vlines,
}
\textbf{Ref.} & \textbf{Year} & \textbf{Data Sources} & \textbf{R} & \textbf{NLP} & \textbf{CTI Type} \\
\cite{shin2021twiti}           & 2021          & SN                    & Y               & NER,TC,KE             & T                 \\
\cite{adewopo2020exploring}        & 2020          & SN,SR,SD,UF           & Y               & TC                    & T                 \\
\cite{zhao2020timiner}           & 2020          & SN,NA,SR,UF,DW        & N               & SA,TC                 & T                 \\
\cite{koloveas2021intime}       & 2021          & SN                    & Y               & NER,SA,TC,KE          & O                 \\
\cite{tekin2021obtaining}          & 2021          & SN                    & Y               & TC                    & T                 \\
\cite{kristiansen2020cti}    & 2020          & SN                    & Y               & TM,TC,KE              & T                 \\
\cite{rodriguez2020enhancing}      & 2020          & SN,NA,SR              & Y               & TM,TC                 & T                 \\
\cite{azevedo2019pure}        & 2019          & FE                    & N               & TM,TC,SU              & T                 \\
\cite{hossen2021generating}        & 2021          & UF                    & Y               & TM,TC                 & T                 \\
\cite{guo2023framework}            & 2023          & FE                    & N               & SU,KE                 & O                 \\
\cite{bose2021tracing}           & 2021          & SN                    & N               & TM,SA                 & O                 \\
\cite{kadoguchi2020deep}     & 2020          & UF                    & Y               & TM                    & T                 \\
\cite{zhou2022cti}           & 2022          & NA,SR                 & N               & NER,KE                & T                 \\
\cite{sakellariou2023secdfan}   & 2023          & OT                    & N               & TM,SA,KE              & T                 \\
\cite{arnold2019dark}        & 2019          & UF,DM                 & Y               & TM,SA,KE              & S                 \\
\cite{tundis2022feature}        & 2022          & SN                    & Y               & SA                    & O                 \\
\cite{cha2020blockchain}           & 2020          & FE                    & N               & SU                    & T                 \\
\cite{ampel2020labeling}         & 2020          & SD,UF,DM              & Y               & TM,TC                 & T                 \\
\cite{purba2023extracting}         & 2023          & SN,SD                 & N               & TC                    & T                 \\
\cite{sun2021automatic}            & 2021          & SR                    & Y               & TC,SU                 & T                 \\
\cite{sufi2023new}          & 2020          & SN,NA,SD              & Y               & TM,SA,TC              & O                 \\
\cite{huang2020monitoring}        & 2019          & UF                    & Y               & TC                    & T                 \\
\cite{zenebe2019cyber}         & 2023          & SN                    & Y               & SA                    & S                 \\
\cite{sufi2023global}           & 2023          & SN,SD                 & N               & SA                    & S                 \\
\cite{furumoto2021extracting}       & 2021          & UF,DM,DW              & Y               & SU                    & T                 \\
\cite{gautam2020hacker}         & 2019          & UF                    & Y               & TC,KE                 & T                 \\
\cite{panagiotou2021towards}    & 2021          & NA                    & Y               & NER,TC                & T                 
\end{tblr}
\caption{Classified papers from the related work. (Note: Ref. = Paper Reference, R = Provided reasons for using specific source(s), NLP = Applied NLP method(s), CTI Type = Extracted CTI type (T = Technical, S = Strategical, O = Operational))}
\label{tab:related}
\end{table}

==> sections/archived/2-background.tex <==
\section{Background}
\label{sec:related}
\noindent
Explain the security-related background of this paper: What is the darknet? Where do cybercriminals communicate? What are typical data sources investigated? Explain how cybercriminals use for instance the Darknet, and also chat channels, e.g. what do they sell. Basically: explain the difference between these ''communication channels'' and social networks, such as Twitter.


In this section, we provide some background information on the sources that we utilized in the proposed approach including Darknet, underground forums, and social networks.

The Darknet can be considered a hidden part of the internet that is not accessible through standard web browsers. To access it, special software such as The Onion Router (TOR), Invisible Internet Project (I2P), and Freenet is necessary. It is a platform for cybercriminals to engage in various illegal activities, including the trade of banned substances, weapons, and stolen data, as well as planning large-scale cyberattacks.

The aspect that we are particularly interested in is the communication between the adversaries. Cybercriminals communicate through underground forums and the aforementioned Darknet websites. These platforms serve as primary sources of information for adversaries to exchange experiences, share information, and plan criminal activities. They offer a wide range of information, illicit goods, and services, including detailed descriptions of specific attacks, hacking tools, malware, breached personal data, and other illegal products. These communication channels accommodate the needs of cybercriminals for anonymity and secure transactions, which enables the Crime-as-a-Service (CaaS) paradigm.

%https://www.sciencedirect.com/science/article/pii/S294979142400023X

On the other hand, social networks such as Telegram and Discord, function as secondary sources of information. While their primary purpose is not solely for criminal activities, these are still widely utilized due to their simplicity and flexibility. These platforms are more versatile and serve multiple purposes beyond criminal activities, including legitimate communication and information sharing.

Besides all of the aforementioned sources being utilized for illegal activities, they also offer fresh and highly relevant intelligence information for cybersecurity practitioners that can be leveraged as cyber threat intelligence (CTI) to enhance an organization's cybersecurity posture. This intelligence can be used to guide strategic and tactical actions to counter cyber threats, concentrating defenses where necessary and maximizing its value to the organization's cybersecurity efforts. Thus, organizations can stay ahead of potential threats, mitigate risks, and protect sensitive data.

\saskia{I am ok with removing the background and adding this part to the introduction, but I don't understand the difference between the primary and secondary sources of information. To me, these are all primary sources of information, and I would consider CTI reports as ''secondary'' sources. In the introduction we should include the following points:}




==> sections/archived/3-data-set.tex <==
%Number of relevant vs. not relevant data items for each data source.


%The English CrimeBB and the Chat dataset come from the same source, as described by Pastrana et al.~\cite{Pastrana2018CrimeBBEC}. Since chat messages and forum posts differ in structure, the data has been grouped into a chat dataset and an English dataset. The English CrimeBB and chat dataset consist of SQL files containing information about pages, members, interactions, ratings, and posts. The CFLW dataset is composed of HTML files crawled from the dark web, each tagged with the main topics by the company CFLW.

%Extracting data from the HTML files was challenging and required additional work compared to the other datasets. The data set is comparatively noisy~\cite{oosthoek2023quantifying}. First, tags considered outside the scope of this paper were filtered out. Tags related to physical goods, such as electronics and drugs, porn, political discussions, and websites under construction were removed. The dataset consists of different snapshots of the same page over time. To avoid re-using the same data multiple times, after the preprocessing step described later, the most recent snapshot of each page was kept~\footnote{Nair et ak.~\cite{nair2021template} highlight the difficulty of identifying duplicate pages on the darknet. Hence, we refrain from identifying duplicates and focus on the most recent content for our analysis.}. %and all previous snapshots of the same page with a normalized Levenshtein distance smaller than twenty per cent were discarded.

%All datasets underwent a preprocessing step, English filtering, and splitting before content analysis. In the preprocessing step, URLs, mentions, tags (words starting with \@ and \#), words containing numbers, and any character not in the English alphabet except for punctuation were removed. Non-ASCII entries were stripped, characters repeating more than three times were cut after the third repetition, lowercase normalization was applied, and contractions were expanded. All text data created before the first of January 2019 was also discarded.

%After preprocessing, an automated English detector was applied to the data. Entries not flagged as English were removed. To eliminate outliers in word count, a splitting procedure was applied. For the English CrimeBB and chat datasets, the maximum total word count was set to 1000, and the word count per row was set to 500. For the CFLW dataset, a maximum total length of 2000 words was used while maintaining a maximum word count per row of 500 words. The CFLW data is generally longer and would lose significant content with a shorter cut-off. Entries with fewer than seven words were dropped as they were considered uninformative.
